Top-k-Convolution and the Quest for Near-Linear Output-Sensitive Subset Sum

In the classical Subset Sum problem we are given a set $X$ and a target $t$, and the task is to decide whether there exists a subset of $X$ which sums to $t$. A recent line of research has resulted in $\tilde{O}(t)$-time algorithms, which are (near-)optimal under popular complexity-theoretic assumptions. On the other hand, the standard dynamic programming algorithm runs in time $O(n \cdot |\mathcal{S}(X,t)|)$, where $\mathcal{S}(X,t)$ is the set of all subset sums of $X$ that are smaller than $t$. Furthermore, all known pseudopolynomial algorithms actually solve a stronger task, since they actually compute the whole set $\mathcal{S}(X,t)$. As the aforementioned two running times are incomparable, in this paper we ask whether one can achieve the best of both worlds: running time $\tilde{O}(|\mathcal{S}(X,t)|)$. In particular, we ask whether $\mathcal{S}(X,t)$ can be computed in near-linear time in the output-size. Using a diverse toolkit containing techniques such as color coding, sparse recovery, and sumset estimates, we make considerable progress towards this question and design an algorithm running in time $\tilde{O}(|\mathcal{S}(X,t)|^{4/3})$. Central to our approach is the study of top-$k$-convolution, a natural problem of independent interest: given sparse polynomials with non-negative coefficients, compute the lowest $k$ non-zero monomials of their product. We design an algorithm running in time $\tilde{O}(k^{4/3})$, by a combination of sparse convolution and sumset estimates considered in Additive Combinatorics. Moreover, we provide evidence that going beyond some of the barriers we have faced requires either an algorithmic breakthrough or possibly new techniques from Additive Combinatorics on how to pass from information on restricted sumsets to information on unrestricted sumsets.

==> more_results.tex <==
\section{Proof of theorems from \ref{subsub:more_results} }

We first prove Theorem \ref{thm:more_1}.

\begin{proof}

Let $A_1$ be the set of the smallest $\left \lceil 100 \epsilon |A| \right \rceil $ numbers in $A$, $A_3$ the set of the largest $\left \lceil 100\epsilon |A| \right \rceil$ numbers in $A$, and $A_2 = A \setminus ( A_1 \cup A_3)$. Let $B_1,B_2,B_3$ be defined in an analogous way for $B$. We shall compute $(A_1 + B) \cap [u,v], (A_3 + B) \cap [u,v], (A+B_1) \cap [u,v], ( A+B_3) \cap [u,v], (A_2 + B_2) \cap [u,v]$. For the first four computations we shall invoke Theorem \ref{thm:interval}. Note that each computation takes time (ignoring $\log $ factors) $\sqrt{ \epsilon |A| \cdot |B| \cdot |(A+B)\cap [u]}$, since in each sumset computation at least one of the sets' sizes is a $O( \epsilon )$ fraction of the size of the initial set it has occurred from. For $(A_2+B_2) \cap [u,v]$ we shall compute $A_2+B_2$ via a standard unrestricted sumset computation, namely Theorem \ref{thm:sparse_convolution}. In what follows we bound $A_2 + B_2$ in terms of $(A+B)\cap [u,v]$.


\begin{enumerate}
\item $\tilde{A} + \tilde{B}$ is totally contained in $[u,v]$, i.e. $(\tilde{A} + \tilde{B}) \cap [u,v] = \tilde{A} + \tilde{B}$,
\item $\tilde{A} + B_2, A_2 + \tilde{B}$ are totally contained in $[u,v]$, and 
\item $|\tilde{A}| = \Omega( |A|), |\tilde{B}| = \Omega( |B|)$. 
\end{enumerate} 

If such sets exist, then applying two times Ruzsa's triangle inequality (Lemma \ref{lem:ruzsa}) we shall obtain

	\[	|A_2 + B_2| \leq \frac{ |A_2 + \tilde{B}| \cdot |\tilde{B} + \tilde{A}| \cdot |\tilde{A} + B_2|}{|\tilde{A}|\cdot |\tilde{B}|} \leq O\left( \frac{|(A+B)\cap [u,v]|^3}{|A||B|}\right).				\]

Thus, from now on we shall focus on proving the existence of these two sets.


First, observe the following. We cannot have that all $a\in A_1$ satisfy $| (\{a\} + B) \cap [0,u-1]| > \frac{|B|}{100}$, otherwise we would have more than $\frac{B}{100} \cdot (100 \epsilon |A|) = \epsilon |A||B|$ pairs $(a,b) \in A \times B$ with $a+b \notin [u,v]$. For that reason, this means that for the largest $a \in A_1$ we have $| (\{a\} + B) \cap \{u,u+1\ldots,\}| \geq \frac{99|B|}{100}$, and thus the same inequality is satisfied for every $a \in A_2$, since everyone in $A_2$ is larger than anyone in $A_1$. The symmetric argument for $A_3$ yields that for everyone in $A_2$ we have that 
$|(\{a\} + B ) \cap [v]| \geq \frac{99|B|}{100}$. Thus, combining both inequalities we obtain that every $a \in A_2$ satisfies $|\{a\} + B \cap [u,v] | \geq \frac{98}{100} |B|$. Now, let $a_m$ (respectively $a_M$) be the smallest (respectively largest) element in $A_2$. Let also $B_m$ be the set of $b \in B$ such that $a_m + b \in [u,v]$, and, similarly $B_M$ the set of $b \in B$ such that $a_M + b \in [u,v]$. It easily follows that $|B_m|, |B_M| \geq \frac{98}{100} |B|$, since $|(\{a_m\} + B) \cap [u,v] |, |(\{a_M\} + B) \cap [u,v] | \geq \frac{98}{100} |B|$. Set $\tilde{B} = |\left(B_m \cap B_M \right) \setminus (B_1 \cup B_2)|$. Then we have the following.
\begin{itemize}
\item $\tilde{B} = \Omega(|B|)$, namely \[|\tilde{B}| \geq \frac{96}{100}|B| - 2 \left \lceil \epsilon |B| \right \rceil \geq \frac{95}{100} |B|,\] since $ |B_m \cap B_M| = |B_m| + |B_M| - |B_m \cup B_M| \geq \frac{98}{100} |B| + \frac{98}{100}|B| - |B| = \frac{96}{100}|B|$, and each of $B_1,B_3$ contains at most $\left \lceil \epsilon |B| \right \rceil$ elements.
\item $ \tilde{B} + A_2$ is totally contained inside $[u,v]$. This holds since $\tilde{B}+ \{a_m\}$ and $\tilde{B} + \{a_M\}$ are totally contained inside $[u,v]$, and thus for every other $a \in A_2$ and every $b \in \tilde{B}$, $a+b$ has to be at least $a_m + \mathrm{min}(\tilde{B}) \geq u$ and at most $a_M + \mathrm{max}(\tilde{B}) \leq v$.
\item $\tilde{B} \subseteq B_2$. This is immediate by the definition of $B_M$.
\end{itemize}

Similarly, we can guarantee the existence of a set $\tilde{A} \subseteq A$ such that$|\tilde{A}| \geq \frac{95}{100}|A|$ and $ \tilde{A} + B_2$ is totally contained inside $[u,v]$.
We have that $\tilde{A} + \tilde{B} \subseteq \tilde{A} + B_2 \subseteq [u,v]$. Thus, sets $\tilde{A},\tilde{B}$ satisfy conditions (1)-(3), which guarantees the running time of our algorithm.

\end{proof}

We now prove Theorem \ref{thm:more_2}.

\Vasileios{to be filled}
\begin{proof}
According to Lemma \ref{lem:conv_promise} we may assume that we solve the IR-SMP problem where we are also given a set $T$ of size $O(|(A+B)\cap [u]|)$ containg $(A+B)\cap [u]$.
Let $A_1$ be the largest $\left \lceil 100 \epsilon |A| \right \rceil $ numbers in $A$, and $B_1$ be the largest $\left \lceil 100 \epsilon |B| \right \rceil $ numbers in $B$. Let $A_2 = A \setminus A_1, B_2 = B \setminus B_1$. Let $y = \frac{|T|^{5/3}}{n} \epsilon^{-\frac{1}{3} }$. Let $i^*$ be the smallest index such that $ | (a_{i^*} +B ) \cap [u])| \leq y$. Similarly let $j^*$ be the smallest index such that $ | (A + b_{j^*} ) \cap [u])| \leq y$. We perform the following sumset computations.

\begin{enumerate}
\item $A_2 + B_2$ via Theorem \ref{thm:sparse_convolution}. Using Lemma \ref{lem:bound_rectangle} the running time 
\[	\frac{|(A_2+B_2)\cap [u]|^3}{100n \cdot 100 n} = O\left( \frac{|(A+B)\cap [u]|}{n^2} \right).	\]

\end{enumerate}



\end{proof}


Lastly, we procceed with the proof of Theorem \ref{thm:more_3}.

\begin{proof}
As we have mentioned before, it suffices to solve the IR-SMP problem, where we also given a set $T$ containing $(A+B)\cap [u]$. By standard arguments, we may assume that $|T|$ is at least an absolute constant. We first shift $A,B$ by a very large number $2M$ to $A''=\{2M\}+A$, $B''=\{2M\}+B$. Then we add the numbers
\[ \{ 1, 3M+u-1, 3M+u-2, ..., 3M+u-|T|\}\]
to both $A''$ and $B''$ to form $A',B'$. We set $u' = 4M+u$, and solve the $(A'',B'',u')$ prefix-restricted sumset computation.
Note that $(3M+|T|-x) + (2M+y) >> u'$, and thus the large added numbers do not interfere with the shifted $A$ and $B$. Thus, the output consists of:
\begin{enumerate}
\item $(A''+B'')\bigcap [u] = \{4M\}+(A+B)\bigcap [u]$,
\item $A'+\{1\}$,
\item $\{1\}+B'$
\end{enumerate}
In particular, we can reconstruct $(A+B)\cap [u]$ given $(A'+B')\cap [u']$. We have $|A'| = 1 + |T| + |A| = \Theta( |A| + |(A+B)\cap [u]|)$, and similarly $|B'| = \Theta(|B| +  |(A+B)\cap [u]|$.
Moreover, the new output size satisfies $ |A+B| \geq |A'+B'| \leq |A+B| + |A'| + |B'| = O(|(A+B)\cap [u])$. Plugging in these bounds, we obtain the desired reduction.

\end{proof}

